Neural Approximate Sufficient Statistics for Implicit Models

We consider the fundamental problem of how to automatically construct summary statistics for implicit generative models where the evaluation of the likelihood function is intractable, but sampling data from the model is possible. The idea is to frame the task of constructing sufficient statistics as learning mutual information maximizing representations of the data with the help of deep neural networks. The infomax learning procedure does not need to estimate any density or density ratio. We apply our approach to both traditional approximate Bayesian computation and recent neural likelihood methods, boosting their performance on a range of tasks.

==> bk/2.methodology-2.tex <==
\section{Methodology}
 

\subsection{Neural sufficient statistics}
Our new deep neural network-based approach for automatic construction of near-sufficient statistics is based on the infomax principle, as illustrated by the following proposition: 
\begin{Proposition}
    Let $\vectheta \sim p(\vectheta)$, $\vecx \sim p(\vecx|\vectheta)$, and $s: \mathcal{X} \to \mathcal{S}$ be a deterministic function. Then $\vecs = s(\vecx)$ is a sufficient statistic for $p(\vecx|\vectheta)$ if and only if 
    \[
        s = \mathop{\arg\max}_{S: \mathcal{X} \to \mathcal{S}} \enskip I(\vectheta; S(X)) ,
    \label{MI-sufficiency}
    \]
    where $S$ is deterministic mapping and $I(\cdot; \cdot)$ is the mutual information between random variables. 
\end{Proposition}

\emph{Proof}. We defer the complete proof to the appendix. This proposition is a variant of Theorem 8 in \citep{Shamir2008Learning} with an adaption to likelihood-free inference scenario. \qed \\

This important result suggests that we could find the sufficient statistic $\vecs = s(\vecx)$ for a likelihood function $p(\vecx|\vectheta)$ by maximizing the mutual information (MI) $I(\vectheta; \vecs) = KL[p(\vectheta, \vecs) \Vert  p(\vectheta)p(\vecs)]$ between $\vectheta$ and $\vecs$.
Moreover, as our interest is in maximizing MI rather than knowing its precise value, we can maximize its non-KL surrogate, which may have advantage in e.g. estimation accuracy or computational efficiency \citep{hjelm2018learning, ozair2019wasserstein, szekely2007measuring}. To this end, we utilize the following two non-KL estimators: 

\if0 To this end, we utilize the Jensen-Shannon divergence (JSD) surrogate \citep{hjelm2018learning}, a distribution-free, non-KL MI estimator. More specifically, it estimates MI as: \fi


\begin{figure*}[t]
\centering
%\vspace{-1cm}
\includegraphics[width=1.0\linewidth]{figures/pipeline2.png}
\caption{
\emph{Left}. Traditional likelihood-free inference algorithm needs handcrafted design of summary statistic, which requires expert knowledge.
\emph{Right}. Our method automatically mines a low dimensional, near-sufficient statistic $\vecs$ of $\vecx$ via infomax principle, which removes the need of careful summary statistic design. Furthermore, this statistic could be re-learned as the posterior inference proceeds. 
}
\label{figure:networks}
\end{figure*}



\textbf{Jensen-Shannon divergence} (JSD)  \citep{hjelm2018learning}: this non-KL estimator is shown to be more robust than KL-based ones. More specifically, it estimates MI as:
\begin{equation}
\hat I^{\text{JSD}}(\vectheta; \vecs) = \sup_{T: \Theta \times \mathcal{S} \to \R}\mathbb{E}_{p(\vectheta, \vecs)}\left[-\operatorname{sp} (-T(\vectheta, \vecs))\right]-\mathbb{E}_{p(\vectheta)p(\vecs)}\left[\operatorname{sp} (T(\vectheta, \vecs)) \right],
\label{formula:MI-JSD}
\end{equation}
where $\operatorname{sp}(t) = \log(1+\exp(t))$ is the softplus function. With this estimator, we set up the following objective for learning the sufficient statistics, which simultaneously estimates and maximizes the MI:
\begin{equation}
\mathcal{L}(S, T) =  \mathbb{E}_{p(\vectheta, \vecx)}\left[-\operatorname{sp}\left(-T(\vectheta; S(\vecx))\right)\right]-\mathbb{E}_{p(\vectheta)p(\vecx)}\left[\operatorname{sp}\left(T(\vectheta; S(\vecx)\right)\right],
\label{formula:obj}
\end{equation}
where the two deterministic mappings $S$ and $T$ are parameterized by two neural networks. Note that we have used the law of the unconscious statistician (LOTUS) from \eqref{formula:MI-JSD} to \eqref{formula:obj}. An empirical version of \eqref{formula:obj} is given in the appendix. 

\textbf{Distance correlation} (DC) \citep{szekely2007measuring}: unlike the JSD estimator, this  estimator does not need to learn an additional network $T$, nor to generate samples $(\vectheta, \vecx) \sim p(\vecx)p(\vectheta)$ (which is time-consuming due to the random permutation operation required in the sampling process), hence can be learned much faster. It estimates MI as:
\newcommand{\DCXY}{\mathbb{E}^2_{p(\vectheta, \vecs)p(\vectheta', \vecs')}[h(\vectheta, \vectheta')h(\vecs, \vecs')]}
\newcommand{\DCXX}{\mathbb{E}_{p(\vectheta)p(\vectheta')}[h^2(\vectheta, \vectheta')]}
\newcommand{\DCYY}{\mathbb{E}_{p(\vecs)p(\vecs')}[h^2(\vecs, \vecs')]}
\begin{equation}
\hat{I}^{\text{DC}}(\vectheta; \vecs) = \frac{\DCXY}{\DCXX \cdot \DCYY},
\label{formula:MI-DC}
\end{equation}
where $h(\veca, \vecb) = \|\veca - \vecb\| - \mathbb{E}_{p(\vecb')}[\|\veca - \vecb'\|] - \mathbb{E}_{p(\veca')}[\|\veca' - \vecb\|] + \mathbb{E}_{p(\veca')p(\vecb')}[\|\veca' - \vecb'\|]$. Similar to the case of JSD estimator, we set up the following objective for learning the sufficient statistics:
\newcommand{\DCxy}{\mathbb{E}^2_{p(\vectheta, \vecx)p(\vectheta', \vecx')}[h(\vectheta, \vectheta')h(S(\vecx), S(\vecx'))]}
\newcommand{\DCxx}{\mathbb{E}_{p(\vectheta)p(\vectheta')}[h^2(\vectheta, \vectheta')]}
\newcommand{\DCyy}{\mathbb{E}_{p(\vecx)p(\vecx')}[h^2(S(\vecx), S(\vecx'))]}
\begin{equation}
    \mathcal{L}(S) = \frac{\DCxy}{\DCxx \cdot \DCyy},
    \label{formula:obj2}
\end{equation}
where the deterministic mapping $S$ is parameterized by a  neural network. Again LOTUS is used from \eqref{formula:MI-DC} to \eqref{formula:obj2}. An empirical version of \eqref{formula:obj2} is given in the appendix. 

We empirically find that the JSD estimator generally yields (slightly) more accurate inference result, whereas the DC estimator has the advantage of much faster execution time (see the appendix for more details). Which estimator to use indeed depends on the demand. In practice, we recommend to use the DC estimator for coarse-grained statistics learning (e.g. early rounds of sequential learning), and use the JSD estimator for fine-grained statistics learning (e.g. the last round of sequential learning). 

\if0 However, since the focus of this paper is to improve inference accuracy, we will mainly report the result based on the JSD estimator in the experiment. \fi

With considerable training samples and powerful neural networks, we could obtain near-sufficient statistic with either $s = \mathop{\arg\max}_{S}\max_T \mathcal{L}(S, T)$  or $s = \mathop{\arg\max}_{S}\mathcal{L}(S)$, depending on the estimator. The statistic $\vecs$ of data $\vecx$ is then given by
% $\vecs = s(\vecx)$.
\begin{equation}
    \vecs = s(\vecx).
\end{equation}
In the above construction, we have not specified the form of the networks $S$ and $T$. For $S$, any prior knowledge about the data $\vecx$ could in principle be incorporated into its design. For example, for sequential data we can realize $S$ as a transformer \citep{vaswani2017attention}, and for exchangeable data we can realize $S$ as a exchangeable neural network \citep{ss-nn-1}. Here we simply adopt a fully-connected architecture for $S$, and leave the problem-specific design of $S$ as future work. For $T$, we choose it to be a split architecture $T(\vectheta; S(\vecx)) = T'(H(\vectheta); S(\vecx))$ where $T'(\cdot, \cdot), H(\cdot)$ are both MLPs. Therefore we separately learn low-dimensional representations for $\vecx$ and $\vectheta$ before processing them together. This could be seen as that we incorporate the inductive bias into the design of the networks that $\vecx$ and $\vectheta$ should \emph{not} interact with each other directly, based on their true relationship (for example, consider the likelihood function of exponential family: $L(\vectheta; \vecx) \propto \text{exp}(H(\vectheta)^{\top}S(\vecx))$). \\

\if0
We are left with the problem of how to select $d$, the dimensionality of the sufficient statistics. The  Pitman-Koopman-Darmois theorem tells us that sufficient statistics with fixed dimensionality only exists for the exponential family, so one might better determine $d$ in a data-driven way. To do this, we can in principle set $d$ to be as low as possible while preserving enough information about $\vectheta$:
\begin{equation}
    d = \min \{d': \hat{I}(s_{d'}(X); \vectheta) \geq  \lambda \hat{I}(s_{d^*}(X); \vectheta) \}
    \label{formula:determine-d}
\end{equation}
where $s_{d'}$ is the statistics with dimensionality $d'$, $d^*$ is the dimensionality that achieves the highest  MI value, $\hat{I}$ is the estimated MI value and $\lambda \in (0,1)$ quantifies how much information we are to preserve in the learned statistics (e.g. $\lambda = 0.975$). For this purpose we can train multiple statistics networks in one loss simultaneously and compare their MI values. Due to space limit we do not pursue this idea further in this paper and leave its verification to future work.
\fi



We are left with the problem of how to select $d$, the dimensionality of the sufficient statistics. The  Pitman-Koopman-Darmois theorem tells us that sufficient statistics with fixed dimensionality only exists for exponential family, so there is no universal way to select $d$. Here, we propose to use the following simple heuristics to determine $d$: 
\begin{equation}
    d = 2K
\end{equation}
where $K$ is the dimensionality of $\vectheta$ (which typically satisfies $K \ll D$). The rationale behind this heuristics is that the dimensionality of the sufficient statistics in exponential family is $K$, and exponential family has been proven reasonably accurate for posterior approximation (see e.g. \citep{thomas2021likelihood, pacchiardi2020score}). Now, by doubling the dimensionality of the statistics to $2K$ we are likely to have better representative power than exponential family while still keeping $d$ small.



Furthermore, we have the following proposition comparing our method to the existing 
\emph{posterior-mean-as-statistic} approaches \citep{ss1, ss3}. \\


\begin{Proposition}
\label{prop:non_sufficiency}
    Let $\vectheta \sim p(\vectheta)$ and $\vecx \sim p(\vecx|\vectheta)$. Let $s(\cdot)$ be the maximizer of the following objective:
    \[
    \label{eq:posterior_mean}
        s = \mathop{\arg\min}_{S: \mathcal{X} \to \mathcal{S}} \enskip \mathbb{E}_{p(\vectheta, \vecx)}[\|S(\vecx) - \vectheta\|^2_2],
    \]
    then $\vecs = s(\vecx)$ is generally not a maximizer of $I(S(\vecx); \vectheta)$ and hence it is not a sufficient statistic.
\end{Proposition}
\emph{Proof}. We defer the proof to the appendix. \qed \\

This proposition tells us that unlike our method, the existing (posterior-)mean-as-statistic approaches widely used in likelihood-free inference community loose information about the posterior, and it is only optimal for predicting the posterior mean \citep{ss1, ss3}. When using this statistics in inference, it may yield inaccurate estimation to e.g. the posterior uncertainty. Nonetheless which statistic to use depends on the task e.g.\ full posterior estimate vs.\ point estimate. 

\if0
\footnote{This does not mean these mean-as-statistics approaches will completely lose information about the posterior uncertainty. For example, different parameters $\vectheta$ can still generate data whose statistics values $\vecs$ are the same.  }
\fi

\if0
In addition to the comparison with the mean-as-statistics approach, one may also compare  statistics to expert statistics and how to select between them. Here, rather than selecting between the learned statistics and the expert statistics, which is difficult, we propose to incorporate them into a \emph{joint} statistics: 
\begin{equation}
    \vecs = [\vecs_{\text{expert}}, s(\vecx)]
\end{equation}
and we feed this joint statistics into the MI estimators (3)(5) to learn $s(\cdot)$. This can be seen as that we learn an `augmented statistics' $s(\vecx)$ to compensate for the non-sufficiency of expert statistics. By doing so, we combine the power of expert knowledge and data-driven learning in the design of summary statistics. No selection is needed. We verify the usefulness of this strategy in the appendix.
\fi









% \begin{minipage}[!t]{0.49\linewidth}
% \centering
% \begin{algorithm}[H]
%   \caption{SMC-ABC+}
%   \label{alg:smc-abc+}
% \begin{algorithmic}
%   \STATE {\bfseries Input:} prior $\pi(\vectheta)$, observed data $\vecx_o$
%   \STATE {\bfseries Output:} estimated posterior $\hat{\pi}(\vectheta|\vecx^o)$
%   \STATE {\bfseries Initialization:} $\mathcal{D} = \varnothing, p_1(\vectheta) = \pi(\vectheta)$
%   \FOR{$j$ in $1$ to $r$ } 
%     %\STATE $\triangleright \enskip$ \emph{Simulation}
%     \REPEAT
%      \STATE sample $\vectheta^{(i)} \sim p_j(\vectheta)$ ; 
%      \STATE simulate $\vecx^{(i)} \sim p(\vecx|\vectheta_i)$ ;
%     \UNTIL{$n$ samples}
%     \STATE $\mathcal{D} \leftarrow \mathcal{D} \cup \{\vectheta_i, \vecx_i\}^{n}_{i=1}$
%     %\STATE
%     %\STATE $\triangleright \enskip $ \emph{Learning}
%     \STATE fit statistic net $s(\cdot)$ with $\mathcal{D}$ by  \eqref{formula:obj} ;
%     \STATE sort $\mathcal{D}$ according to $\|s(\vecx_i) - s(\vecx_o)\|$ ;
%     \STATE fit $ p(\vectheta|\vecs_o)$ with the top $m$ $\vectheta$s in $\mathcal{D}$;
%     \STATE $q_j(\vectheta|\vecs_o) \propto \pi(\vectheta)/\sum_j p_j(\vectheta) \cdot  p(\vectheta|\vecs_o)$;
%     \STATE $p_{j+1}(\vectheta) \leftarrow q_{j}(\vectheta|\vecs_o)$;
%     \vspace{0.04cm}
%   \ENDFOR 
%   \STATE \textbf{return} $\hat{\pi}(\vectheta|\vecx_o) = q_{r}(\vectheta|\vecs_o)$
% \end{algorithmic}
% \end{algorithm}
% \vspace{0.1cm}
% \end{minipage}%
% \hspace{+0.01\linewidth}
% \begin{minipage}[!t]{0.49\linewidth}
% \begin{algorithm}[H]
%   \caption{SNL+}
%   \label{alg:snl+}
% \begin{algorithmic}
%   \STATE {\bfseries Input:} prior $\pi(\vectheta)$, observed data $\vecx_o$
%   \STATE {\bfseries Output:} estimated posterior $\hat{\pi}(\vectheta|\vecx^o)$
%   \STATE {\bfseries Initialization:} $\mathcal{D} = \varnothing, p_1(\vectheta) = \pi(\vectheta)$
%   \FOR{$j$ in $1$ to $r$ } 
%     %\STATE $\triangleright \enskip$ \emph{Simulation}
%     \REPEAT
%      \STATE sample $\vectheta^{(i)} \sim p_j(\vectheta)$ ; 
%      \STATE simulate $\vecx^{(i)} \sim p(\vecx|\vectheta_i)$ ;
%     \UNTIL{$n$ samples}
%     \STATE $\mathcal{D} \leftarrow \mathcal{D} \cup \{\vectheta_i, \vecx_i\}^{n}_{i=1}$
%     %\STATE 
%     %\STATE $\triangleright \enskip $ \emph{Learning}
%     \STATE fit statistic net $s(\cdot)$ with $\mathcal{D}$ by  \eqref{formula:obj};
%     \STATE convert $\mathcal{D}$ with the learned $s(\cdot)$;
%     \STATE fit $q(\vecs|\vectheta)$ with converted $\mathcal{D}$ by \eqref{formula:SNL};
%     \STATE $q_j(\vectheta|\vecs_o) \propto \pi(\vectheta) \cdot q(\vecs_o|\vectheta)$;
%     \STATE $p_{j+1}(\vectheta) \leftarrow q_{j}(\vectheta|\vecs_o)$;
%     \vspace{0.04cm}
%   \ENDFOR 
%   \STATE \textbf{return} $\hat{\pi}(\vectheta|\vecx_o) = q_{r}(\vectheta|\vecs_o)$
% \end{algorithmic}
% \end{algorithm}
% \vspace{0.1cm}
% \end{minipage}


\subsection{Dynamic statistic learning}
The above neural sufficient statistic could, in principle, be learned via a pilot run before the inference starts, as typically done in the work by \citet{ss2, ss1, ss3}. Such a strategy requires extra simulation cost, and the learned statistic is kept fixed during inference. We propose a dynamic learning strategy below to overcome these limitations. 


Our idea is to \textit{jointly learn the statistic and the posterior in multiple rounds}. More concretely, at round $r$, we use the current statistic $s(\cdot)$ to build the $r$-th estimate to the posterior: $q_r(\vectheta|\vecs_o)  \approx \pi(\vectheta|\vecx_o)$, whereas at round $r$+1, this estimate is used as the new proposal distribution to simulate data: $ p_{r+1}(\vectheta) \gets q_r(\vectheta|\vecs_o), \vectheta_i \sim p_{r+1}(\vectheta), \vecx_i \sim p(\vecx|\vectheta_i)$. We then re-learn $s(\cdot)$ and $q(\cdot)$ with all the data up to the new round. In this process, $s(\cdot)$ and $q(\cdot)$ refine each other: a good $s(\cdot)$ helps to learn $q(\cdot)$ more accurately, whereas an improved $q(\cdot)$ as a better proposal in turn helps to learn $s(\cdot)$ more efficiently. 

The theoretical basis of this multi-rounds strategy is provided by Proposition 1, which essentially tells that a different $p(\vectheta)$ will \emph{not} affect the sufficiency of the learned statistics. This means that we are safe to use any proposal distribution $p_j(\vectheta)$ at any round $j$ (and in this case $p(\vectheta) = \frac{1}{r}\sum^r_j p_j(\vectheta)$). 




\if0
One may wonder if the learned statistics is still sufficient in the above multi-rounds strategy. This is answered by Proposition 1 which essentially tells that a different marginal distribution $p(\vectheta)$ for $\vectheta$ in the sampled data $\mathcal{D} = \{\vecx_i, \vectheta_i \}^{nr}_{i=1}$ will \emph{not} affect the sufficiency of the learned statistics, namely
\begin{equation}
    \mathop{\arg\max}_{S} KL[p(\vectheta, S(\vecx)) \Vert  p(\vectheta)p(S(\vecx))] = \mathop{\arg\max}_{S} KL[p'(\vectheta, S(\vecx)) \Vert  p'(\vectheta)p(S(\vecx))]
\end{equation}
where $p(\vectheta) \neq p'(\vectheta)$. Therefore we are safe to use any proposal $p_j(\vectheta)$ in any round $j$ during learning. 
\fi



\begin{minipage}[!t]{0.49\linewidth}
\centering
\begin{algorithm}[H]
  \caption{SMC-ABC+}
  \label{alg:smc-abc+}
\begin{algorithmic}
  \STATE {\bfseries Input:} prior $\pi(\vectheta)$, observed data $\vecx_o$
  \STATE {\bfseries Output:} estimated posterior $\hat{\pi}(\vectheta|\vecx^o)$
  \STATE {\bfseries Initialization:} $\mathcal{D} = \varnothing, p_1(\vectheta) = \pi(\vectheta)$
  \FOR{$j$ in $1$ to $r$ } 
    %\STATE $\triangleright \enskip$ \emph{Simulation}
    \REPEAT
     \STATE sample $\vectheta^{(i)} \sim p_j(\vectheta)$ ; 
     \STATE simulate $\vecx^{(i)} \sim p(\vecx|\vectheta_i)$ ;
    \UNTIL{$n$ samples}
    \STATE $\mathcal{D} \leftarrow \mathcal{D} \cup \{\vectheta_i, \vecx_i\}^{n}_{i=1}$
    %\STATE
    %\STATE $\triangleright \enskip $ \emph{Learning}
    \STATE fit statistic net $s(\cdot)$ with $\mathcal{D}$ by  \eqref{formula:obj} ;
    %\STATE (optional) select between $s$, $s_{\text{expert}}$ by MI;
    \STATE sort $\mathcal{D}$ according to $\|s(\vecx_i) - s(\vecx_o)\|$ ;
    \STATE fit $ p(\vectheta|\vecs_o)$ with the top $m$ $\vectheta$s in $\mathcal{D}$;
    \STATE $q_j(\vectheta|\vecs_o) \propto \pi(\vectheta)/\sum_j p_j(\vectheta) \cdot  p(\vectheta|\vecs_o)$;
    \STATE $p_{j+1}(\vectheta) \leftarrow q_{j}(\vectheta|\vecs_o)$;
    \vspace{0.04cm}
  \ENDFOR 
  \STATE \textbf{return} $\hat{\pi}(\vectheta|\vecx_o) = q_{r}(\vectheta|\vecs_o)$
\end{algorithmic}
\end{algorithm}
\vspace{0.1cm}
\end{minipage}%
\hspace{+0.01\linewidth}
\begin{minipage}[!t]{0.49\linewidth}
\begin{algorithm}[H]
  \caption{SNL+}
  \label{alg:snl+}
\begin{algorithmic}
  \STATE {\bfseries Input:} prior $\pi(\vectheta)$, observed data $\vecx_o$
  \STATE {\bfseries Output:} estimated posterior $\hat{\pi}(\vectheta|\vecx^o)$
  \STATE {\bfseries Initialization:} $\mathcal{D} = \varnothing, p_1(\vectheta) = \pi(\vectheta)$
  \FOR{$j$ in $1$ to $r$ } 
    %\STATE $\triangleright \enskip$ \emph{Simulation}
    \REPEAT
     \STATE sample $\vectheta^{(i)} \sim p_j(\vectheta)$ ; 
     \STATE simulate $\vecx^{(i)} \sim p(\vecx|\vectheta_i)$ ;
    \UNTIL{$n$ samples}
    \STATE $\mathcal{D} \leftarrow \mathcal{D} \cup \{\vectheta_i, \vecx_i\}^{n}_{i=1}$
    %\STATE 
    %\STATE $\triangleright \enskip $ \emph{Learning}
    \STATE fit statistic net $s(\cdot)$ with $\mathcal{D}$ by  \eqref{formula:obj};
    %\STATE (optional) select between $s$, $s_{\text{expert}}$ by MI;
    \STATE convert $\mathcal{D}$ with the learne $s(\cdot)$;
    \STATE fit $q(\vecs|\vectheta)$ with converted $\mathcal{D}$ by \eqref{formula:SNL};
    \STATE $q_j(\vectheta|\vecs_o) \propto \pi(\vectheta) \cdot q(\vecs_o|\vectheta)$;
    \STATE $p_{j+1}(\vectheta) \leftarrow q_{j}(\vectheta|\vecs_o)$;
    \vspace{0.04cm}
  \ENDFOR 
  \STATE \textbf{return} $\hat{\pi}(\vectheta|\vecx_o) = q_{r}(\vectheta|\vecs_o)$
\end{algorithmic}
\end{algorithm}
\vspace{0.1cm}
\end{minipage}


In practice, any likelihood-free inference algorithm that learns the posterior sequentially naturally fits well within the above joint statistic-posterior learning strategy. Here we study two such instances:


\textbf{Sequential Monte Carlo ABC (SMC-ABC)} \citep{smc-abc}. This classical algorithm learns the posterior in a non-parametric way within multiple rounds. Here, we consider a variant of it to better make use of the above neural sufficient statistic, and to re-use all previous simulated data. The new SMC-ABC algorithm estimates the posterior $q_r(\vectheta|\vecs_o)$ at the $r$-th round as follows. We first sort data in $\mathcal{D} = \{\vecx_i, \vectheta_i \}^{nr}_{i=1}$ according to the distances $\|s(\vecx_i) - s(\vecx_o)\|$. We then pick the top-$m$ $\vectheta$s whose corresponding distances are the smallest. The picked $\vectheta$s then follow $\vectheta \sim p(\vectheta \mid\vecs_o)$ as below:
\begin{equation}
    p(\vectheta\mid\vecs_o) \propto \sum^r_{j=1} p_j(\vectheta) \cdot \text{Pr}(\|\vecs - \vecs_o \|<\epsilon \mid \vectheta),
    \label{formula:SMC-ABC}
\end{equation}
where the threshold $\epsilon$ is implicitly defined by the ratio $\frac{m}{nr}$ (which automatically goes to zero as $r \to \infty$). We then fit $p(\vectheta|\vecs_o)$ with the collected $\vectheta$s by a flexible parametric model (e.g. a Gaussian copula), with which we can obtain the $r$-th estimate to the posterior by importance (re-)weighting:
\begin{equation}
    q_r(\vectheta\mid\vecs_o) \propto \pi(\vectheta)/{\sum^r_{j=1} p_j(\vectheta)} \cdot p(\vectheta\mid\vecs_o).
\end{equation}
\if0 To further improve performance, we apply \emph{model averaging} when returning the posterior estimate. More specifically, rather than directly taking $\hat{\pi}(\vectheta|\vecx_o) = q_r(\vectheta|\vecs_o)$, we take it as the average of the recent $m$ estimates: $\hat{\pi}(\vectheta|\vecx_o) = \frac{1}{m} \sum^{m}_{t=0} q_{r-t}(\vectheta|\vecs_o)$. Here we simply set $m=3$, which as we confirm empirically achieves good performance. By doing so, we as if have trained multiple $s(\cdot)$ when estimating $\pi(\vectheta|\vecs_o)$. 
The whole procedure of the new algorithm, SMC-ABC+, is in Algorithm \ref{alg:smc-abc+}. \fi
The whole procedure of this new inference algorithm, SMC-ABC+, is summarized in Algorithm \ref{alg:smc-abc+}.



\textbf{Sequential Neural Likelihood (SNL)} \citep{papamakarios2019sequential}. This recent algorithm learns the posterior in a parametric way, also in multiple rounds. The original SNL method approximates the likelihood function $p(\vecx|\vectheta)$ by a conditional neural density estimator $q(\vecx|\vectheta)$, which could be difficult to learn if the dimensionality of $\vecx$ is  high. Here, we alleviate such difficulty with our neural statistic. The new SNL algorithm estimates the posterior $q_r(\vectheta|\vecs_o)$  at the $r$-th round as follows. At round $r$, where we have $nr$ simulated data $\mathcal{D}= \{\vectheta_i, \vecx_i \}^{nr}_{i=1}$, we fit a neural density estimator $q(\vecs|\vectheta)$ as:
\begin{equation}
    q({\vecs\mid\vectheta}) = \mathop{\arg\max}_{Q} \sum_{i=1}^{nr} \log Q(s(\vecx_i)\mid\vectheta_i),
    \label{formula:SNL}
\end{equation}
where $s(\cdot)$ is the current statistic network. With $nr$ being moderately large, this would yield us $q(\vecs|\vectheta) \approx p(\vecs|\vectheta)$. We then obtain the $r$-th estimate of the posterior by Bayes rule:
\begin{equation}
q_r(\vectheta\mid\vecs^o) \propto \pi(\vectheta) \cdot q(\vecs^o\mid\vectheta).
\end{equation} 
\if0 Similar to SMC-ABC+, to further improve inference quality, we also employ model averaging with 
the recent $m$ estimates when returning the estimated posterior: $\hat{\pi}(\vectheta|\vecx_o) = \frac{1}{m} \sum^{m}_{t=0} q_{r-t}(\vectheta|\vecs_o)$. The whole procedure of this new SNL algorithm, denoted as SNL+, is summarized in Algorithm  \ref{alg:snl+}. \fi
The whole procedure of this new SNL algorithm, denoted as SNL+, is summarized in Algorithm  \ref{alg:snl+}.


==> bk/2.methodology.tex <==
\section{Methodology}
 

\subsection{Neural sufficient statistics}
Our new deep neural network-based approach for automatic construction of (near-)sufficient statistics is based on the infomax principle, as illustrated by the following proposition 
% (please also see \cite{Shamir2008Learning} for a related result)
: 
\begin{Proposition}
    Let $\vectheta \sim p(\vectheta)$, $\vecx \sim p(\vecx|\vectheta)$, and $s: \mathcal{X} \to \mathcal{S}$ be a deterministic function. Then $\vecs = s(\vecx)$ is a sufficient statistic for $p(\vecx|\vectheta)$ if and only if 
    \[
        s = \mathop{\arg\max}_{S: \mathcal{X} \to \mathcal{S}} \enskip I(\vectheta; S(X)) ,
    \label{MI-sufficiency}
    \]
    where $S$ is deterministic mapping and $I(\cdot; \cdot)$ is the mutual information between random variables. 
\end{Proposition}

\emph{Proof}. We defer the complete proof to the Appendix. This proposition is a variant of Theorem 8 in \citep{Shamir2008Learning} with an adaption to likelihood-free inference scenario. \qed

This important result suggests that we could find the sufficient statistic $s(\vecx)$ for a likelihood function $p(\vecx|\vectheta)$ by maximizing the mutual information (MI) $I(\vectheta; S) = KL[p(\vectheta, S) \Vert  p(\vectheta)p(S)]$ between $\vectheta$ and $S$.
Moreover, as our interest is in maximizing MI rather than knowing its precise value, we can maximize a non-KL surrogate, which has been proven to yield better performance \citep{hjelm2018learning, ozair2019wasserstein, wen2020mutual}. To this end, we utilize the Jensen-Shannon divergence (JSD) surrogate \citep{hjelm2018learning}, a distribution-free, non-KL MI estimator. This estimator was shown to be much less sensitive to sample size \citep{hjelm2018learning}. More specifically, it estimates MI as:
\begin{equation}
\hat I^{\text{JSD}}(\vectheta; S) = \sup_{T: \Theta \times \mathcal{S} \to \R}\mathbb{E}_{p(\vectheta, \vecs)}\left[-\operatorname{sp} (-T(\vectheta, \vecs))\right]-\mathbb{E}_{p(\vectheta)p(\vecs)}\left[\operatorname{sp} (T(\vectheta, \vecs)) \right],
\label{formula:MI-JSD}
\end{equation}
where $\operatorname{sp}(t) = \log(1+\exp(t))$ is the softplus function. With this estimator, we set up the following objective for learning the sufficient statistics, which simultaneously estimates and maximizes the MI:
\begin{equation}
\mathcal{L}(S, T) =  \mathbb{E}_{p(\vectheta, \vecx)}\left[-\operatorname{sp}\left(-T(\vectheta; S(\vecx))\right)\right]-\mathbb{E}_{p(\vectheta)p(\vecx)}\left[\operatorname{sp}\left(T(\vectheta; S(\vecx)\right)\right],
\label{formula:obj}
\end{equation}
\if0
To this end, we utilize the Wasserstein distance (WD) surrogate \citep{ozair2019wasserstein}, a distribution-free, non-KL MI estimator. It estimates MI as:
\begin{equation}
\hat I^{\text{WD}}(\vectheta; S) = \sup_{\| T\|_L \leq 1}\mathbb{E}_{p(\vectheta, \vecs)}\left[T(\vectheta, \vecs)\right]-\mathbb{E}_{p(\vectheta)p(\vecs)}\left[ T(\vectheta, \vecs) \right],
\label{formula:MI-JSD}
\end{equation}
where $T: \Theta \times \mathcal{S} \to \R$ is a 1-Lipschitz function. With this estimator, we set up the following objective for learning the sufficient statistic, which imultaneously estimates and maximizes the MI:
\begin{equation}
\begin{gathered}
\max \mathcal{L}(S, T) =  \mathbb{E}_{p(\vectheta, \vecx)}\left[T(\vectheta; S(\vecx))\right]-\mathbb{E}_{p(\vectheta)p(\vecx)}\left[T(\vectheta; S(\vecx))\right], \\
s.t
\quad \|\nabla_{\vectheta, \vecs}T(\vectheta , \vecs)\|_2 \leq 1
\end{gathered}
\label{formula:obj}
\end{equation}
\fi
where the two deterministic mappings $S$ and $T$ are parameterized by two neural networks. \if0Note that we have used the law of the unconscious statistician from \eqref{formula:MI-JSD} to \eqref{formula:obj}.\fi \if0 The 1-Lipschitz constraint could be implemented by e.g gradient penalty \citep{gulrajani2017improved}. \fi

With considerable training samples and powerful neural networks $S$ and $T$, we could obtain near-sufficient statistic with $s = \mathop{\arg\max}_{S}\max_T \mathcal{L}(S, T)$. The statistic $\vecs$ of data $\vecx$ is then given by
% $\vecs = s(\vecx)$.
\begin{equation}
    \vecs = s(\vecx).
\end{equation}
In the above construction, we have not specified the form of the networks $S$ and $T$. For $T$, we choose it to be a split architecture: 
\begin{equation}
    T(\vectheta; S(\vecx)) = T'(H(\vectheta); S(\vecx)),
\end{equation}
where $T'(\cdot, \cdot), H(\cdot)$ are both MLPs.  For $S$, any prior knowledge about the data $\vecx$ could in principle be incorporated into its design. For example, for sequential data  we can realize $S$ as a LSTM network \citep{gers1999learning}, and for exchangeable data  we can realize $S$ as a exchangeable neural network \citep{ss-nn-1}. Here we simply adopt a fully-connected architecture for $S$, and leave the problem-specific design of $S$ as future work. Therefore we separately learn representations for $\vecx$ and $\vectheta$ before processing them together. This could be seen as that we incorporate the inductive bias into the design of the networks that $\vecx$ and $\vectheta$ should \emph{not} interact with each other directly, based on their true relationship, (for example, consider the exponential family: $L(\vectheta; \vecx) \propto \text{exp}(H(\vectheta)^{\top}S(\vecx))$). 

\if0 The  architecture (6) could be seen as a generalization of  the exponential family where we replace $H(\vectheta)^{\top}S(\vecx)$ by $\text{MLP}(H(\vectheta), S(\vecx))$). \fi

We are left with the problem of how to select $d$, the dimensionality of the sufficient statistics. The  Pitman-Koopman-Darmois theorem tells us that sufficient statistics with fixed dimensionality only exists for exponential family, so one might better determine $d$ in a data-driven way. To do this, we can in principle set $d$ to be as low as possible while preserving enough information about $\vectheta$:
\begin{equation}
    d = \min \{d': \hat{I}(s_{d'}(X); \vectheta) \geq  \lambda \hat{I}(s_{d^*}(X); \vectheta) \}
\end{equation}
where $s_{d'}$ is the statistic with dimensionality $d'$, $d^*$ is the dimensionality that achieves the highest MI and $\lambda \in (0,1)$ quantifies how much information we are to preserve in the learnt statistics. \if0 This idea can be realized easily by making the output of $S$ multi-head, with each head corresponding to each dimensionality $d'$ and a distinct $T$ network. We can then jointly train these networks by an aggregation loss:  $\mathcal{L}(S, T) = \sum_{d'}\mathcal{L}_{d'}(S_{d'}, T_{d'})$ where $S_{d'}$ and $T_{d'}$ are the networks for dimensionality $d'$.  \fi Due to space limit we do not pursue this idea further in this paper and leave its verification to future work.

Furthermore, we have the following proposition comparing our method to the existing 
\emph{posterior-mean-as-statistic} approaches \citep{ss1, ss3}.


\begin{Proposition}
\label{prop:non_sufficiency}
    Let $\vectheta \sim p(\vectheta)$ and $\vecx \sim p(\vecx|\vectheta)$. Let $s(\cdot)$ be the maximizer of the following objective:
    \[
    \label{eq:posterior_mean}
        s = \mathop{\arg\min}_{S: \mathcal{X} \to \mathcal{S}} \enskip \mathbb{E}_{p(\vectheta, \vecx)}[\|S(\vecx) - \vectheta\|^2_2],
    \]
    then $\vecs = s(\vecx)$ is generally not a maximizer of $I(S(\vecx); \vectheta)$ and hence it is not a sufficient statistic.
\end{Proposition}
\emph{Proof}. We defer the proof to the Appendix. \qed

This proposition tells us that unlike our method, the existing posterior-mean-as-statistic approaches widely used in likelihood-free inference community loose information about the posterior, and it is only optimal for predicting the posterior mean \citep{ss1, ss3}. Nonetheless which method to use depends on the task e.g.\ full posterior estimate vs.\ point estimate).


\if0 Under some further restriction, this is sometimes referred as \textit{linear sufficiency} \citep{witting1987linear, mueller1987sufficiency}, and is only optimal for predicting the posterior mean. \fi




% \begin{minipage}[!t]{0.49\linewidth}
% \centering
% \begin{algorithm}[H]
%   \caption{SMC-ABC+}
%   \label{alg:smc-abc+}
% \begin{algorithmic}
%   \STATE {\bfseries Input:} prior $\pi(\vectheta)$, observed data $\vecx_o$
%   \STATE {\bfseries Output:} estimated posterior $\hat{\pi}(\vectheta|\vecx^o)$
%   \STATE {\bfseries Initialization:} $\mathcal{D} = \varnothing, p_1(\vectheta) = \pi(\vectheta)$
%   \FOR{$j$ in $1$ to $r$ } 
%     %\STATE $\triangleright \enskip$ \emph{Simulation}
%     \REPEAT
%      \STATE sample $\vectheta^{(i)} \sim p_j(\vectheta)$ ; 
%      \STATE simulate $\vecx^{(i)} \sim p(\vecx|\vectheta_i)$ ;
%     \UNTIL{$n$ samples}
%     \STATE $\mathcal{D} \leftarrow \mathcal{D} \cup \{\vectheta_i, \vecx_i\}^{n}_{i=1}$
%     %\STATE
%     %\STATE $\triangleright \enskip $ \emph{Learning}
%     \STATE fit statistic net $s(\cdot)$ with $\mathcal{D}$ by  \eqref{formula:obj} ;
%     \STATE sort $\mathcal{D}$ according to $\|s(\vecx_i) - s(\vecx_o)\|$ ;
%     \STATE fit $ p(\vectheta|\vecs_o)$ with the top $m$ $\vectheta$s in $\mathcal{D}$;
%     \STATE $q_j(\vectheta|\vecs_o) \propto \pi(\vectheta)/\sum_j p_j(\vectheta) \cdot  p(\vectheta|\vecs_o)$;
%     \STATE $p_{j+1}(\vectheta) \leftarrow q_{j}(\vectheta|\vecs_o)$;
%     \vspace{0.04cm}
%   \ENDFOR 
%   \STATE \textbf{return} $\hat{\pi}(\vectheta|\vecx_o) = q_{r}(\vectheta|\vecs_o)$
% \end{algorithmic}
% \end{algorithm}
% \vspace{0.1cm}
% \end{minipage}%
% \hspace{+0.01\linewidth}
% \begin{minipage}[!t]{0.49\linewidth}
% \begin{algorithm}[H]
%   \caption{SNL+}
%   \label{alg:snl+}
% \begin{algorithmic}
%   \STATE {\bfseries Input:} prior $\pi(\vectheta)$, observed data $\vecx_o$
%   \STATE {\bfseries Output:} estimated posterior $\hat{\pi}(\vectheta|\vecx^o)$
%   \STATE {\bfseries Initialization:} $\mathcal{D} = \varnothing, p_1(\vectheta) = \pi(\vectheta)$
%   \FOR{$j$ in $1$ to $r$ } 
%     %\STATE $\triangleright \enskip$ \emph{Simulation}
%     \REPEAT
%      \STATE sample $\vectheta^{(i)} \sim p_j(\vectheta)$ ; 
%      \STATE simulate $\vecx^{(i)} \sim p(\vecx|\vectheta_i)$ ;
%     \UNTIL{$n$ samples}
%     \STATE $\mathcal{D} \leftarrow \mathcal{D} \cup \{\vectheta_i, \vecx_i\}^{n}_{i=1}$
%     %\STATE 
%     %\STATE $\triangleright \enskip $ \emph{Learning}
%     \STATE fit statistic net $s(\cdot)$ with $\mathcal{D}$ by  \eqref{formula:obj};
%     \STATE convert $\mathcal{D}$ with the learned $s(\cdot)$;
%     \STATE fit $q(\vecs|\vectheta)$ with converted $\mathcal{D}$ by \eqref{formula:SNL};
%     \STATE $q_j(\vectheta|\vecs_o) \propto \pi(\vectheta) \cdot q(\vecs_o|\vectheta)$;
%     \STATE $p_{j+1}(\vectheta) \leftarrow q_{j}(\vectheta|\vecs_o)$;
%     \vspace{0.04cm}
%   \ENDFOR 
%   \STATE \textbf{return} $\hat{\pi}(\vectheta|\vecx_o) = q_{r}(\vectheta|\vecs_o)$
% \end{algorithmic}
% \end{algorithm}
% \vspace{0.1cm}
% \end{minipage}


\subsection{Dynamic statistic-posterior learning}
The above neural sufficient statistic could, in principle, be learned via a pilot run before the inference starts, as typically done in the work by \citet{ss2, ss1, ss3}. Such a strategy requires extra simulation cost, and the learned statistic is kept fixed during inference. We propose a dynamic learning strategy below to overcome these limitations. 


Our idea is to \textit{jointly learn the statistic and the posterior in multiple rounds}. More concretely, at round $r$, we use the current statistic $s(\cdot)$ to build the $r$-th estimate to the posterior: $q_r(\vectheta|\vecs_o)  \approx \pi(\vectheta|\vecx_o)$,  \begin{minipage}[!t]{0.49\linewidth}
\centering
\begin{algorithm}[H]
  \caption{SMC-ABC+}
  \label{alg:smc-abc+}
\begin{algorithmic}
  \STATE {\bfseries Input:} prior $\pi(\vectheta)$, observed data $\vecx_o$
  \STATE {\bfseries Output:} estimated posterior $\hat{\pi}(\vectheta|\vecx^o)$
  \STATE {\bfseries Initialization:} $\mathcal{D} = \varnothing, p_1(\vectheta) = \pi(\vectheta)$
  \FOR{$j$ in $1$ to $r$ } 
    %\STATE $\triangleright \enskip$ \emph{Simulation}
    \REPEAT
     \STATE sample $\vectheta^{(i)} \sim p_j(\vectheta)$ ; 
     \STATE simulate $\vecx^{(i)} \sim p(\vecx|\vectheta_i)$ ;
    \UNTIL{$n$ samples}
    \STATE $\mathcal{D} \leftarrow \mathcal{D} \cup \{\vectheta_i, \vecx_i\}^{n}_{i=1}$
    %\STATE
    %\STATE $\triangleright \enskip $ \emph{Learning}
    \STATE fit statistic net $s(\cdot)$ with $\mathcal{D}$ by  \eqref{formula:obj} ;
    %\STATE (optional) select between $s$, $s_{\text{expert}}$ by MI;
    \STATE sort $\mathcal{D}$ according to $\|s(\vecx_i) - s(\vecx_o)\|$ ;
    \STATE fit $ p(\vectheta|\vecs_o)$ with the top $m$ $\vectheta$s in $\mathcal{D}$;
    \STATE $q_j(\vectheta|\vecs_o) \propto \pi(\vectheta)/\sum_j p_j(\vectheta) \cdot  p(\vectheta|\vecs_o)$;
    \STATE $p_{j+1}(\vectheta) \leftarrow q_{j}(\vectheta|\vecs_o)$;
    \vspace{0.04cm}
  \ENDFOR 
  \STATE \textbf{return} $\hat{\pi}(\vectheta|\vecx_o) = q_{r}(\vectheta|\vecs_o)$
\end{algorithmic}
\end{algorithm}
\vspace{0.1cm}
\end{minipage}%
\hspace{+0.01\linewidth}
\begin{minipage}[!t]{0.49\linewidth}
\begin{algorithm}[H]
  \caption{SNL+}
  \label{alg:snl+}
\begin{algorithmic}
  \STATE {\bfseries Input:} prior $\pi(\vectheta)$, observed data $\vecx_o$
  \STATE {\bfseries Output:} estimated posterior $\hat{\pi}(\vectheta|\vecx^o)$
  \STATE {\bfseries Initialization:} $\mathcal{D} = \varnothing, p_1(\vectheta) = \pi(\vectheta)$
  \FOR{$j$ in $1$ to $r$ } 
    %\STATE $\triangleright \enskip$ \emph{Simulation}
    \REPEAT
     \STATE sample $\vectheta^{(i)} \sim p_j(\vectheta)$ ; 
     \STATE simulate $\vecx^{(i)} \sim p(\vecx|\vectheta_i)$ ;
    \UNTIL{$n$ samples}
    \STATE $\mathcal{D} \leftarrow \mathcal{D} \cup \{\vectheta_i, \vecx_i\}^{n}_{i=1}$
    %\STATE 
    %\STATE $\triangleright \enskip $ \emph{Learning}
    \STATE fit statistic net $s(\cdot)$ with $\mathcal{D}$ by  \eqref{formula:obj};
    %\STATE (optional) select between $s$, $s_{\text{expert}}$ by MI;
    \STATE convert $\mathcal{D}$ with the learned/selected $s(\cdot)$;
    \STATE fit $q(\vecs|\vectheta)$ with converted $\mathcal{D}$ by \eqref{formula:SNL};
    \STATE $q_j(\vectheta|\vecs_o) \propto \pi(\vectheta) \cdot q(\vecs_o|\vectheta)$;
    \STATE $p_{j+1}(\vectheta) \leftarrow q_{j}(\vectheta|\vecs_o)$;
    \vspace{0.04cm}
  \ENDFOR 
  \STATE \textbf{return} $\hat{\pi}(\vectheta|\vecx_o) = q_{r}(\vectheta|\vecs_o)$
\end{algorithmic}
\end{algorithm}
\vspace{0.1cm}
\end{minipage}
whereas at round $r$+1, this estimate is used as the new proposal distribution to simulate data: $ p_{r+1}(\vectheta) \gets q_r(\vectheta|\vecs_o), \vectheta_i \sim p_{r+1}(\vectheta), \vecx_i \sim p(\vecx|\vectheta_i)$. We then re-learn $s(\cdot)$ and $q(\cdot)$ with all the data up to the new round. In this process, $s(\cdot)$ and $q(\cdot)$ refine each other: a good $s(\cdot)$ helps to learn $q(\cdot)$ more accurately, whereas an improved $q(\cdot)$ as a better proposal in turn helps to learn $s(\cdot)$ more efficiently. 







In practice, any likelihood-free inference algorithm that learns the posterior sequentially naturally fits well within the above joint statistic-posterior learning framework. Here we study two such instances:




\textbf{Sequential Monte Carlo ABC (SMC-ABC)} \citep{smc-abc}. This classical algorithm learns the posterior in a non-parametric way within multiple rounds. Here, we consider a variant of it to better make use of the above neural sufficient statistic, and to re-use all previous simulated data. The new SMC-ABC algorithm estimates the posterior $q_r(\vectheta|\vecs_o)$ at the $r$-th round as follows. We first sort data in $\mathcal{D} = \{\vecx_i, \vectheta_i \}^{nr}_{i=1}$ according to the distances $\|s(\vecx_i) - s(\vecx_o)\|$. We then pick the top-$m$ $\vectheta$s whose corresponding distances are the smallest. The picked $\vectheta$s then follow $\vectheta \sim p(\vectheta \mid\vecs_o)$ as below:
\begin{equation}
    p(\vectheta\mid\vecs_o) \propto \sum^r_{j=1} p_j(\vectheta) \cdot \text{Pr}(\|\vecs - \vecs_o \|<\epsilon \mid \vectheta),
    \label{formula:SMC-ABC}
\end{equation}
where the threshold $\epsilon$ is implicitly defined by the ratio $\frac{m}{nr}$ (which automatically goes to zero as $r \to \infty$). We then fit $p(\vectheta|\vecs_o)$ with the collected $\vectheta$s by a flexible parametric model (e.g. a Gaussian copula), with which we can obtain the $r$-th estimate to the posterior by importance (re-)weighting:
\begin{equation}
    q_r(\vectheta\mid\vecs_o) \propto \pi(\vectheta)/{\sum^r_{j=1} p_j(\vectheta)} \cdot p(\vectheta\mid\vecs_o).
\end{equation}
\if0 To further improve performance, we apply \emph{model averaging} when returning the posterior estimate. More specifically, rather than directly taking $\hat{\pi}(\vectheta|\vecx_o) = q_r(\vectheta|\vecs_o)$, we take it as the average of the recent $m$ estimates: $\hat{\pi}(\vectheta|\vecx_o) = \frac{1}{m} \sum^{m}_{t=0} q_{r-t}(\vectheta|\vecs_o)$. Here we simply set $m=3$, which as we confirm empirically achieves good performance. By doing so, we as if have trained multiple $s(\cdot)$ when estimating $\pi(\vectheta|\vecs_o)$. 
The whole procedure of the new algorithm, SMC-ABC+, is in Algorithm \ref{alg:smc-abc+}. \fi
The whole procedure of the new inference algorithm, SMC-ABC+, is summarized in Algorithm \ref{alg:smc-abc+}.



\textbf{Sequential Neural Likelihood (SNL)} \citep{papamakarios2019sequential}. This recent algorithm learns the posterior in a parametric way, also in multiple rounds. The original SNL method approximates the likelihood function $p(\vecx|\vectheta)$ by a conditional neural density estimator $q(\vecx|\vectheta)$, which could be difficult to learn if the dimensionality of $\vecx$ is  high. Here, we alleviate such difficulty with our neural statistic. The new SNL algorithm estimates the posterior $q_r(\vectheta|\vecs_o)$  at the $r$-th round as follows. At round $r$, where we have $nr$ simulated data $\mathcal{D}= \{\vectheta_i, \vecx_i \}^{nr}_{i=1}$, we fit a neural density estimator $q(\vecs|\vectheta)$ as:
\begin{equation}
    q({\vecs\mid\vectheta}) = \mathop{\arg\max}_{Q} \sum_{i=1}^{nr} \log Q(s(\vecx_i)\mid\vectheta_i),
    \label{formula:SNL}
\end{equation}
where $s(\cdot)$ is the current statistic network. With $nr$ being moderately large, this would yield us $q(\vecs|\vectheta) \approx p(\vecs|\vectheta)$. We then obtain the $r$-th estimate of the posterior by Bayes rule:
\begin{equation}
q_r(\vectheta\mid\vecs^o) \propto \pi(\vectheta) \cdot q(\vecs^o\mid\vectheta).
\end{equation} 
\if0 Similar to SMC-ABC+, to further improve inference quality, we also employ model averaging with 
the recent $m$ estimates when returning the estimated posterior: $\hat{\pi}(\vectheta|\vecx_o) = \frac{1}{m} \sum^{m}_{t=0} q_{r-t}(\vectheta|\vecs_o)$. The whole procedure of this new SNL algorithm, denoted as SNL+, is summarized in Algorithm  \ref{alg:snl+}. \fi
The whole procedure of this new SNL algorithm, denoted as SNL+, is summarized in Algorithm  \ref{alg:snl+}.


==> bk/3.related_works.tex <==
\section{Related Works}




% \textbf{Approximate Bayesian computation}. LFI is techniques for inference in statistic models without evaluating their likelihood functions. An earlier line of approach is approximate Bayesian computation (ABC), which works by repeatedly simulating data from the model, and picks those data similar to the observed data to estimate the posterior (\citep{RejABC, mcmc-abc, mcmc-abc2, smc-abc, smc-abc2}. To measure the similarity to the observed data sensibly, it is often wise to use low-dimensional summary statistic rather than the raw data. Apart from ABC, a recent line of approach employs neural density estimators to learn the intractable likelihood (e.g SNL \citep{papamakarios2019sequential, lueckmann2019likelihood}) or directly the posterior (e.g SNPE \citep{papamakarios2016fast, lueckmann2017flexible, greenberg2019automatic}). No similarity is needed to compute in this method. In this work, we show that compact, near-sufficient statistic learned from data could improve both lines of approaches.


\textbf{Approximate Bayesian computation}. ABC denotes techniques for likelihood-free inference which work by repeatedly simulating data from the model and picking those data similar to the observed data to estimate the posterior \citep{Sisson2018}. Naive ABC performs simulation with the prior, whereas advanced variants like MCMC-ABC \citep{mcmc-abc, mcmc-abc2} and SMC-ABC \citep{smc-abc, smc-abc2} perform simulation with informed proposals. To measure the similarity to the observed data sensibly, it is often wise to use low-dimensional summary statistic rather than the raw data in ABC. Here we develop a way to learn compact sufficient statistic for ABC. 

\textbf{Neural density estimator-based inference}. Apart from ABC, a recent line of research uses a conditional neural density estimator to (sequentially) learn the intractable likelihood (e.g SNL \citet{papamakarios2019sequential, lueckmann2019likelihood}) or directly the posterior (e.g SNPE \citet{papamakarios2016fast, lueckmann2017flexible, greenberg2019automatic}). Likelihood-targeting approaches has the advantage that they could readily make use of any proposal distribution in sequential learning, but rely on low-dimensional, well-chosen summary statistic. Posterior-targeting methods on the contrary need no design of summary statistic, but they require non-trivial  efforts to facilitate sequential learning. Our approach (e.g SNL+) could be seen as taking the advantages from both worlds. 


\textbf{Automatic construction of summary statistics}. A set of works have been proposed to automatically construct low-dimensional summary statistics.
% based on different criteria. 
Two lines of them are most related to our approach. The first line \citep{ss1} and its variants \citep{ss3, ss-nn-1,ss-nn-2, ss-nn-3} train a neural network to predict the posterior mean and use this prediction as the summary statistic. These mean-as-statistic approaches, as analyzed previously in Proposition \ref{prop:non_sufficiency}, indeed do not guarantee sufficiency. Rather than taking the predicted mean, the works \citep{alsing2018massive, brehmer2020mining} take the score function $\nabla_{\vectheta} \log p(\vecx|\vectheta)|_{\vectheta = \vectheta^*}$ around some fiducial parameter $\vectheta^*$ as the summary statistic. However, these score-as-statistic approaches are only \emph{locally} sufficient
around $\vectheta^*$, and it requires to first identify $\vectheta^*$ which could itself be difficult. 
Our approach differs from all these methods as it is \emph{globally} sufficient for all $\vectheta$. 
\if0 Methods that targets at global sufficiency does exist \citep{ss4}, but it requires a pre-defined pool of candidate statistic. Our approach differs from all these approaches as we can extract \emph{globally} (near-)sufficient statistic from raw data directly. \fi


\textbf{MI and ratio estimation}. It has been shown in the literature that many variational MI estimators $I(X; Y)$ also estimate the ratio $p(X, Y)/p(X)p(Y)$ up to a constant \citep{nowozin2016f, Nguyen_2010}. Therefore our MI-based statistic learning method is closely related to ratio estimation approaches like \citep{cranmer2015approximating, thomas2016likelihood, hermans2019likelihood}. The differences are  1) we estimate the ratio in the low-dimensional space rather than in the original space by a particular network architecture, based on a sufficient statistics perspective; 2) we decouple the task of statistic learning from the task of density estimation, which grants us the privilege to use any infomax representation learning methods that are ratio-free, e.g. \citet{ozair2019wasserstein, szekely2007measuring}.


==> bk/4.experiments.tex <==
\section{Experiments}
\subsection{Setup}

\textbf{Baselines}. We apply the proposed  statistic to two aforementioned likelihood-free inference methods: (i) SMC-ABC \citep{smc-abc} (the slightly modified version) and (ii) SNL \citep{papamakarios2019sequential}. We compare the performance of the algorithms augmented with our neural statistics (dubbed as SMC-ABC+ and SNL+) to their original versions as well as the versions based on expert-designed statistics (details presented later; we call the corresponding methods SMC-ABC' and SNL'). We also compare to the sequential neural posterior estimate (SNPE) method \footnote{More specifically, the version B. We select to compare with SNPE-B \citep{lueckmann2017flexible} rather than the more recent SNPE-C \citep{greenberg2019automatic} due to its similarity to SRE shown in \citep{durkan2020contrastive}.} which needs no statistic design, as well as the sequential ratio estimate (SRE) method \citep{hermans2019likelihood} which is  closely related to our MI-based method\footnote{For fair comparison, we control that the neural network in SRE has the similar number of parameters/same optimizer settings as in our method. See the appendix for more details about the settings of the neural networks.}. All methods are run for 10 rounds with 1,000 simulations each.



% the popular regression based summary statistic method [1,2], which uses the estimated posterior mean $\hat{\mathbb{E}}[\vectheta|\vecx^o]$ as the summary statistic. We apply these methods to two likelihood-free inference methods: (a) Sequential Monte Carlo-ABC (SMC-ABC) [1], a traditional ABC approach which learns the posterior in multiple rounds. For this method, we simulate 1000 samples per round, and pick the top 200\% samples closest to $\vecx_o$ of the current population to estimate posterior. The proposal distribution is updated after each round using these samples. (b) Sequential Neural Likelihood (SNL) [5], a state-of-the-art approach based on neural density estimator. For this method, which also learns posterior in multiple rounds, we simulate 1000 samples per round, and re-estimate the posterior after each round. \if0 This is the same setting as in [5]. \fi


\textbf{Evaluation metric}. To assess the quality of the estimated posterior, we compare the Jensen-Shannon divergence (JSD) between the approximate posterior $Q$ and the true posterior $P$ in each method:
% The JSD between $P$ and $Q$ is defined as:
\[
    \text{JSD}(P, Q) = \frac{1}{2} \text{KL}[P\|(Q+P)/2] +  \frac{1}{2}\text{KL}[Q\|(Q+P)/2] 
\]
For the problems we consider in the experiments, the true posterior $P$ is either analytically available, or could be accurately approximated by a standard rejection ABC algorithm \citep{RejABC}. \if0 with known low-dimensional sufficient statistic (e.g $s(\vecx) \in \Z$) and extensive simulations (e.g $10^6$).  See more details in supplementary materials. \fi
% The calculation of JSD is done numerically by a Riemann sum over $30^K$ equally spaced grids with $K$ being the dimensionality of $\vectheta$. The region of these grids is jointly defined by  the samples from $P$ and $Q$. For inference methods that only return samples of the posterior (e.g SMC-ABC), we estimate $Q$ by Gaussian copula, as has been done in \cite{gc-abc, gc-abc2, chen2019adaptive}. 


\begin{figure*}[t]
\label{fig:ising}
    \hspace{-0.02\linewidth}
    \begin{subfigure}{.35\textwidth}
            \centering
            \vspace{0.46cm}
            \label{fig:ising-a}
            \begin{minipage}[t]{0.70\linewidth}
            \centering
            \includegraphics[width=1.0\linewidth]{figures/IS/ising_data.png}
            \end{minipage}
            \vspace{0.45cm}
            \caption{ }
    \end{subfigure}
    \hspace{-0.06\linewidth}
    \begin{subfigure}{.35\textwidth}
            \centering
            \label{fig:ising-b}
            \begin{minipage}[t]{1.\linewidth}
            \centering
            \includegraphics[width=1.0\linewidth]{figures/IS/IS_result_new.eps}
            \end{minipage}
            \caption{ }
    \end{subfigure}
    \hspace{-0.02\linewidth}
    \begin{subfigure}{.35\textwidth}
            \centering
            \label{fig:ising-c}
            \begin{minipage}[t]{1.0\linewidth}
            \centering
            \includegraphics[width=1.0\linewidth]{figures/IS/stat_comparison.png}
            \end{minipage}
            \caption{ }
    \end{subfigure}
    \caption{\textbf{Ising model}. (a) The 64D observed data $\vecx_o \in \{-1,1\}^{64}$. (b) The JSD between the true and the learned posteriors. (c) The relationship between the learned statistics and the sufficient statistic. }
\end{figure*}

% \vspace{-0.2cm}
\begin{table}[t]
  \label{op-table}
  \centering
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{cccccc}
    \toprule
    % \cmidrule(r){1-5}
    \cmidrule(r){1-6}
%   \textbf{SMC'}  & \textbf{SMC+}    &  \textbf{SNL'} & \textbf{SNL+} & \textbf{SRE} \\
{SMC'}  & {SMC+}    &  {SNL'} & {SNL+} & {SRE}
& {SNPE}
\\
    \midrule
    $0.008 \pm 0.006$  & $0.046 \pm 0.051$  & $0.007 \pm 0.002$   &  $0.015$ $\pm 0.011$  &  $0.083 \pm 0.029$  & $0.058 \pm 0.039$  \\
    \bottomrule
  \end{tabular}
  }
  \caption{\textbf{Ising model}. The JSD between the learned and true posterior with 10,000 simulations. Here SMC' and SNL' utilize the ground-truth sufficient statistics guided by human prior knowledge.
}
\end{table}


\subsection{Results}
We demonstrate the effectiveness of our method in three cases: (a) an Ising model; (b) a  Gaussian copula model; (c) an Ornstein-Uhlenbeck process.
The Ising model does not have an analytical likelihood but the posterior can be approximated accurately by rejection ABC due to the existence of low-dimensional, discrete sufficient statistic. \if0 We also use this model to verify whether our learned statistic is sufficient. \fi The last two models have analytical likelihoods and hence analytical posteriors.
\if0 The dimensionality of the raw data in these models are designed to be high ($D \geq 40$).\fi  These models cover the cases of graph data, i.i.d data and sequence data.\footnote{We chose to conduct experiments on these models rather than common tasks like M/G/1 and Lotka-Volterra since they lack a known true likelihood, making it hard to verify the sufficiency of the proposed statistics. How to evaluate LFI methods on models without known likelihood is still an open problem \citep{lueckmann2021benchmarking}.}


\if0 and are very representative in real-world applications \fi 



\textbf{Ising model}. The first model we consider is a mathematical model in statistical physics that describes the states of atomic spins on a $8 \times 8$ lattice (see Figure~1(a)). Each spin has two states described by a discrete random variable $x_i \in \{-1, +1\}$, and is only allowed to interact with its neighbour. Given parameters $\vectheta = \{\theta_1, \theta_2 \}$, the probability density function of the Ising model is:
\[
  p(\vecx|\vectheta) \propto e^{-H(\vecx; \vectheta)},
\]
\[
  H(\vecx; \vectheta) = - \theta_1 \sum_{\langle i,j \rangle} x_i x_j - \theta_2 \sum_i x_i. 
\]
where $\langle i,j \rangle$ denotes that spin $i$ and spin $j$ are neighbours. $H$ is also called the Hamiltonian of the model. Here, the likelihood function of this model is not analytical due to the intractable normalizing constant $Z(\vectheta) = \sum_{\vecx \in \{-1,1\}^{m\cdot m}} e^{-H(\vecx; \vectheta)}$. However, sampling from the model by MCMC is possible. Note that the sufficient statistic is known for this model: $s^*(\vecx) = \{ \sum_{\langle i,j \rangle} x_i x_j, \sum_i x_i \}$. The true posterior in this model can easily be approximated by a rejection ABC algorithm run with this low-dimensional sufficient statistic and extensive simulations. Here, we assume that $\theta_2$ is known, and the task is to infer the posterior of $\theta_1$ under an uniform prior $\theta_1 \sim \mathcal{U}(0, 1.5)$ (in this case the sufficient statistic becomes only 1D: $s^*(\vecx) = \sum_{\langle i,j \rangle} x_i x_j$). The true parameters are $\vectheta^* = \{0.3, 0.1\}$. 

In Figure 1(c), we investigate whether the proposed statistic could achieve sufficiency. Ideally, if the learned statistic $s$ in our method does recover the true sufficient statistic $s^*$ well, the relationship between $s$ and $s^*$ should be nearly monotonic (note that both $s$ and $s^*$ here are 1D). To verify this, we plot the relationship between $s^*$ and $s$. We see from the figure that $s$ learned in our method does increase monotonically with $s^*$ approximately, suggesting that $s$ recovers $\vecs^*$ reasonably well. In comparison, the statistics learned in the widely-used posterior-mean-as-statistics approach only has weak dependence on the true sufficient statistic; it is nearly indistinguishable for different $s^*$. In other words, it loses sufficiency. The result also verifies our previous theoretical result in Proposition 2. 

Figure 1(b) further shows the JSD between the true and learned posterior for different methods across the rounds (the vertical lines indicates standard errors, each JSD is obtained by calculating the average of 3 independent runs. The results shown in the below experiments have the same setup). It can be seen from the figure that for this model, likelihood-free inference methods augmented with the proposed statistic (SMC-ABC+, SNL+)  outperform their original counterparts (SMC-ABC, SNL) by a large margin. In Table 1, we further compare our statistics with the expert designed statistics, from which one can see their close performance (here the expert statistics is taken as the true sufficient statistics $\vecs^*$). We also see that our method also seems to outperform SRE which directly estimates the ratio $t(\vecx, \vectheta) = p(\vecx, \vectheta)/p(\vecx)p(\vectheta) \propto L(\vectheta; \vecx)$ in high-dimensional space (note that the true likelihood is actually of the form $L(\vectheta; \vecx) = \exp(\vectheta s^*(\vecx))/Z(\vectheta)$) as well as SNPE (version B). The reason why SNPE(-B) does not perform more satisfactorily might be that it relies on importance weights to facilitate sequential learning, which can induce high variance that makes the training unstable.



\if0
Figure 1(b) further shows the JSD between the true and estimation posterior for the different methods under different simulation budgets (the vertical lines indicates standard errors, each JSD is obtained by calculating the average of 5 independent runs. The results shown in the below experiments have the same setup). It can be seen from the figure that for this model, likelihood-free inference methods augmented with the proposed neural sufficient statistic (SMC-ABC+, SNL+)  outperforms their original counterparts (SMC-ABC, SNL) by a large margin. This is because the dimensionality $D$ of the original data $\vecx$ in this problem is very high ($D=64$), so that  SMC-ABC can not sensibly measure the distance between the data and the observed data, and vanilla SNL encounters difficulties when trying to model the  high-dimensional likelihood $p(\vecx|\vectheta)$ given the $n=10^4$ training data. Our neural sufficient statistic alleviates such difficulties, bringing consistent improvements for both methods. 
\fi






% \vspace{20pt}
% \begin{wrapfigure}{r}{0.25\textwidth}  
% % \hspace{-0.01\textwidth}
% \vspace{-5pt}
% \includegraphics[width=.25\textwidth]{figures/GC/GC_data.png}
% \vspace{-15pt}
% % \caption{Observed 2D GC data}
% \caption{GC data}
% % \vspace{-0pt}
% % \label{fig:c}
% \end{wrapfigure}
% \vspace{-25pt}


\begin{figure*}[t]
    \hspace{-0.02\linewidth}
    \begin{subfigure}{.35\textwidth}
            \centering
            \label{fig:gc-a}
            \begin{minipage}[t]{1.0\linewidth}
            \centering
            \includegraphics[width=1.0\linewidth]{figures/GC/GC_data.png}
            \end{minipage}
            \caption{ }
    \end{subfigure}
    \hspace{-0.04\linewidth}
    \begin{subfigure}{.35\textwidth}
            \centering
            \label{fig:gc-b}
            \begin{minipage}[t]{1.0\linewidth}
            \centering
            \includegraphics[width=1.0\linewidth]{figures/GC/GC_result_new.eps}
            \end{minipage}
            \caption{ }
    \end{subfigure}
    \hspace{-0.04\linewidth}
    \begin{subfigure}{.35\textwidth}
            \centering
            \label{fig:gc-c}
            \vspace{9pt}
            \begin{minipage}[t]{1.0\linewidth}
            \centering
            \hspace{-10pt}
            \tiny
            \begin{tabular}{ccc}
              \includegraphics[width=0.30\linewidth]{figures/GC/GC_theta01_true.png} &
              \hspace{-14pt}
              \includegraphics[width=0.30\linewidth]{figures/GC/GC_smc_round10_theta01_jsd016.png} &  
              \hspace{-14pt}
              \includegraphics[width=0.30\linewidth]{figures/GC/GC_smc2_round10_theta01_jsd01.png} \\
              Truth & SMC \enskip & SMC+ \enskip  \\
              \includegraphics[width=0.30\linewidth]{figures/OP/empty.png}
              &
              \hspace{-14pt}
             \includegraphics[width=0.30\linewidth]{figures/GC/GC_snl_round10_theta01_jsd022.png} &  
             \hspace{-14pt}
             \includegraphics[width=0.30\linewidth]{figures/GC/GC_snl2_round10_theta01_jsd004.png} \\
              & SNL \enskip & SNL+ \enskip  \\
            \end{tabular}
            \end{minipage}
            \caption{ }
    \end{subfigure}
    \caption{\textbf{Gaussian copula}. (a) The observed data $\vecx_o$ in this problem, which is comprised of a population of 200 i.i.d samples. (b) The JSD between the true/learned posteriors. (c) The contours. }
\end{figure*}


% \vspace{-0.2cm}
\begin{table}[t]
  \label{gc-table}
  \centering
  \resizebox{\textwidth}{!}{
  \begin{tabular}{cccccc}
    \toprule
    \cmidrule(r){1-6}
%   \textbf{SMC'}  & \textbf{SMC+}    &  \textbf{SNL'} & \textbf{SNL+} & \textbf{SRE} \\
   {SMC'}  & {SMC+}    &  {SNL'} & {SNL+} & {SRE} & SNPE \\
    \midrule
    $0.183 \pm 0.014 $  & $0.047 \pm 0.009$  & $0.054 \pm 0.016$   & $0.042 \pm 0.006$  &  $0.052 \pm 0.032$  &  $0.037 \pm 0.018$  \\
    \bottomrule
  \end{tabular}
  }
  \caption{\textbf{Gaussian copula}. The JSD between the learned and true posterior with 10,000 simulations. Here SMC' and SNL' utilize the hand-crafted summary statistics guided by human prior knowledge.
}
\end{table}

 
 

 


\textbf{Gaussian copula}. The second model we consider is a 2D Gaussian copula model \citep{chen2019adaptive}. Data $\vecx$ in this model can be seen as generated from the latent variable $\vecz$ as follows:
\[
    \vecz \sim \mathcal{N}\Big(\vecz; \mathbf{0}, \begin{bmatrix}
          1, & \theta_3 \\
          \theta_3, & 1\\
         \end{bmatrix} \Big),
\]
% \[
%     \vecu = \Phi(\vecz),
% \]
\[
   x_1 = F_1^{-1}(\Phi(z_1); \theta_1), \quad x_2 = F_2^{-1}(\Phi(z_2); \theta_2),
\]
\[
    f_1(x_1;\theta_1) = \text{Beta}(x_1; \theta_1, 2), \quad 
    f_2(x_2;\theta_2) = \theta_2 \mathcal{N}(x_2; 1, 1) + (1-\theta_2) \mathcal{N}(x_2; 4, 1/4).
\]
where $\Phi(\cdot)$, $F_1(x_1;\theta_1)$, $F_2(x_2;\theta_2)$ are the cumulative distribution function (CDF) of standard normal distribution, the CDF of $f_1(x_1;\theta_1)$ and the CDF of $f_2(x_2;\theta_2)$ respectively. We assume that a total number of 200 samples are i.i.d drawn from this model, yielding a population $\mathbf{X} = \{\vecx_i\}^{200}_{i=1}$ that serves as our observed data. 
\if0 Note that the likelihood of this model can be computed analytically as $p(\vecx|\vectheta) = c_G(\vecu; \theta_3)  f(x_1;\theta_1)f(x_2;\theta_2)$ where $c_G$ is the Gaussian copula density \citep{gc-abc, chen2019adaptive}. \fi Note that the likelihood of this model can be computed analytically by the law of variable transformation. To perform inference, we compute a rudimentary statistic to describe $\mathbf{X}$, namely (a) the 20-equally spaced quantiles of the marginal distributions of $\mathbf{X}$ and (b) the correlation between the latent variables $z_1, z_2$ in $\mathbf{X}$, resulting in a statistic of dimensionality 41. \if0 This statistic, albeit rudimentary, captures most information about $\mathbf{X}$. This low-level statistic is then treated as the data in LFI algorithms. \fi An uniform prior is set: $\theta_1 \sim \mathcal{U}(0.5, 12.5), \theta_2 \sim \mathcal{U}(0, 1), \theta_3 \sim \mathcal{U}(0.4, 0.8)$ and \if0 the true parameters are $\vectheta^* = \{6,0.5,0.6\}$. \fi $\vectheta^* = \{6,0.5,0.6\}$.

In Figure 2(b), we demonstrate the power of our neural sufficient statistic learning method on the Gaussian copula problem. Overall, we see that the proposed method improves the accuracy of existing likelihood-free inference methods, as well as their robustness (see e.g the reduced variability in SNL+. The high variability in SNL may be due to the lack of training data required to learn the 41-dimensional likelihood function well). This is also confirmed by the contours plots in Figure 2(c). In Table 2 we further compare the proposed statistic with the expert-designed low-dimension statistic (here the expert statistic is taken to be the $5$-equally spaced marginal quantiles + the correlations between $z_1, z_2$), from which we see that our proposed statistic achieves a better performance. For this model, our method seems to perform slightly worse than SNPE (possibly due to the imperfect infomax learning on this problem), but the gap there is indeed very small ($\leq 0.005$ JSD). \if0 We conjecture that more reliable infomax learning methods might help to resolve this issue. \fi





\if0
In Figure 2(b),  we demonstrate the power of our neural sufficient statistic learning method onthe Gaussian copula problem.  Overall, we see that the proposed method significantly boosts theperformance of existing likelihood-free inference methods, no matter on traditional ABC-basedmethod or modern neural density estimator-based method. no matter on traditional ABC-based method or modern neural density estimator-based method. Notably, the proposed method also has an additional effect on improving the robustness, especially for the case of SNL (see e.g the reduced variability in SNL+. The high variability in SNL may be due to the lack of training data required to learn the 41-dimensional likelihood function well). Figure 2(c) further compares the contours of the true posterior and the estimated posteriors in each method. It can be observed from the plots that the posteriors built on the proposed learnt statistic is clearly more accurate as well as more reasonable.
\fi


% We conduct all experiments for 10 rounds and 1,000 simulations within each round and compare the Jensen-Shannon divergence between the estimated posterior of each method and ground truth posterior. The experimental result shows that the proposed method could effectively boost the performance of original methods, no matter traditional ABC based-methods or modern deep learning-based methods. Every data point is estimated from three independent runs as before. We can observe that our method has an extra variance reduction effect compared to vanilla version, corroborating the effectiveness of our jointly learning method. The right part plots the learned posterior contour of distributions of parameter $\vectheta$, indicating the posterior built on proposed learnt statistic could fix the over screwy tendency of SMC-ABC and SNL to some extent and generate more accurate posterior.





\begin{figure*}[t]
    \hspace{-0.02\linewidth}
    \begin{subfigure}{.35\textwidth}
            \centering
            \label{fig:op-a}
            \begin{minipage}[t]{1.0\linewidth}
            \centering
            \includegraphics[width=1.0\linewidth]{figures/OP/OP_data.png}
            \end{minipage}
            \caption{ }
    \end{subfigure}
    \hspace{-0.04\linewidth}
    \begin{subfigure}{.35\textwidth}
            \centering
            \label{fig:op-b}
            \begin{minipage}[t]{1.0\linewidth}
            \centering
            \includegraphics[width=1.0\linewidth]{figures/OP/OP_result_new.eps}
            \end{minipage}
            \caption{ }
    \end{subfigure}
    \hspace{-0.04\linewidth}
    \begin{subfigure}{.35\textwidth}
            \centering
            \label{fig:op-c}
            \vspace{9pt}
            \begin{minipage}[t]{1.0\linewidth}
            \centering
            \hspace{-10pt}
            \tiny
            \begin{tabular}{ccc}
              \includegraphics[width=0.29\linewidth]{figures/OP/OP_theta_true.png} &
              \hspace{-14pt}
              \includegraphics[width=0.30\linewidth]{figures/OP/OP_smc_round10.png} &  
              \hspace{-14pt}
              \includegraphics[width=0.30\linewidth]{figures/OP/OP_smc2_round10.png} \\
              Truth & SMC \enskip & SMC+ \enskip  \\
              \includegraphics[width=0.30\linewidth]{figures/OP/empty.png}
              &
              \hspace{-14pt}
             \includegraphics[width=0.30\linewidth]{figures/OP/OP_snl_round4_jsd004.png} &  
             \hspace{-14pt}
             \includegraphics[width=0.280\linewidth]{figures/OP/OP_snl2_round10_jsd0001.png} \\
              & SNL \enskip & SNL+ \enskip  \\
            \end{tabular}
            \end{minipage}
            \caption{ }
    \end{subfigure}
    \caption{\textbf{OU process}. (a) The observed time-series data $\vecx_o = \{x_t\}^{50}_{t=1}$. (b) The JSD between the true and the learned posteriors. (c) The contours of the true posterior and the learned posteriors. }
\end{figure*}

% \vspace{-0.2cm}
\begin{table}[t]
  \label{op-table}
  \centering
  \resizebox{\textwidth}{!}{
  \begin{tabular}{cccccc}
    \toprule
    \cmidrule(r){1-6}
    % \cmidrule(r){1-6}
%   \textbf{SMC'}  & \textbf{SMC+}    &  \textbf{SNL'} & \textbf{SNL+} & \textbf{SRE} & \textbf{SNP} \\
       {SMC'}  & {SMC+}    &  {SNL'} & {SNL+} & {SRE} 
      & {SNPE} 
       \\
    \midrule
    $ 0.040 \pm 0.006 $  & $ 0.044 \pm 0.018 $  & $ 0.004 \pm 0.001  $   & $ 0.009 \pm 0.002  $  &  $ 0.022 \pm 0.013 $
    & $ 0.019 \pm 0.009 $   
    \\
    \bottomrule
  \end{tabular}
  }
  \caption{\textbf{OU process}. The JSD between the learned and the true posterior with 10,000 simulations. Here SMC' and SNL' utilize the hand-crafted summary statistics guided by human prior knowledge.
}
\end{table}

% \subsection{Ornstein-Uhlenbeck process}
\textbf{Ornstein-Uhlenbeck process}. 
The last model we consider is a stochastic differential equation (SDE). Data $\vecx = \{x_t\}^{D}_{t=1}$ in this model is sequentially generated as:
\[
    x_{t+1} = x_t + \Delta x_t,
\]
\[
    \Delta x_t = \theta_1(\text{exp}(\theta_2) - x_t) \Delta t + 0.5 \epsilon, \quad \epsilon \sim \mathcal{N}(\epsilon; 0, \Delta t).
\]
where $D = 50$, $\Delta t=0.2$ and $x_0=10$. This SDE can be simulated by Euler-Maruyama method, and has an analytical likelihood. \if0 $p(\vecx|\vectheta) = \prod^n_{t=1} p(x_t|x_{t-1}, \vectheta) = \prod^D_{t=1} \mathcal{N}(x_t; \mu_t, \sigma_t)$ in which $\mu_t = x_{t-1} + \theta_1(\text{exp}(\theta_2)-x_{t-1})\Delta t$ and $\sigma_i = 0.5\sqrt{\Delta_t}$. \fi It has a wide applications in financial mathematics and physical sciences. Here, the parameters of interest are $\vectheta = \{\theta_1, \theta_2\}$, and a uniform prior is placed on these parameters: $\theta_1 \sim \mathcal{U}(0, 1), \theta_1 \sim \mathcal{U}(-2.0, 2.0)$. The true parameters are set to be $\vectheta^* = \{0.5, 1.0\}$. 


Figure 3(b) compares the JSD of each method against the simulation cost. Again, we find that the proposed neural sufficient statistics greatly improves the performance of both SMC-ABC and SNL. \if0 not only for accuracy but also for robustness (see the reduced variability in both SMC-ABC+ and SNL+). This can also be confirmed from the contour plots in Figure 3(c). These contour plots also serve as a useful proxy for demonstrating the sufficiency of the learned statistic in our method, as the contours in SMC-ABC+ and SNL+ are highly similar to the contour of  true posterior. \fi In Table 3, we compare our statistics to expert statistic (here the expert statistics are taken as the mean, standard error and autocorrelation with lag 1, 2, 3 of the time series). It can be seen that our statistics are comparable to the expert statistics. Our method also seems to outperform SRE and SNPE. 



\if0
Figure 3.(b) compares the JSD of each method v.s different simulation cost. Again, we find that the proposed neural sufficient statistics greatly improve the performance of both SMC-ABC and SNL, not only for accuracy but also for robustness (see the reduced variability in both SMC-ABC+ and SNL+). In Figure 3.(c), we further visualize the contours of the learned posteriors in each method, from which one can confirm the better inference quality of SMC-ABC+ and SNL+. These contour plots also serve as a useful proxy for demonstrating the sufficiency of the learned statistic in our method, as the contours in SMC-ABC+ and SNL+ are highly similar to the contour of  true posterior.  
\fi











==> bk/_bk.tex <==
% In order to eliminate the negative effect due to the possibly inaccurate estimate of $q_r(\vectheta|\vecs_o)$ in the above adaptive learning strategy, we further develop a new robust proposal distribution. Rather than directly taking the proposal distribution as $p_r(\vectheta) = q_{r-1}(\vectheta|\vecs_o)$, we take $p_r(\vectheta)$ as follows:
% \begin{equation}
%     p_r(\vectheta) \propto \begin{cases} 1 &\mbox{if }  q_{r-1}(\vectheta|\vecs_o) \geq t \\ 
%  q_{r-1}(\vectheta|\vecs_o) & \mbox{if }  q_{r-1}(\vectheta|\vecs_o) < t \end{cases}
%  \label{formula:robust-proposal}
% \end{equation}
% where $t$ is a threshold that distinguish between the `high density region' and `low density region' of $q_{r-1}(\vectheta|\vecs_o)$. Here, we simply set $t$ to be the $50\%$ quantile of the density of $q_{r-1}(\vectheta|\vecs_o)$ values. Therefore $p_r(\vectheta)$ would be uniform at the high density region of $q_{r-1}(\vectheta|\vecs_o)$ and would be proportional to $q_{r-1}(\vectheta|\vecs_o)$ at the low density region. The rationale behind this proposal distribution is two folds: 
% \begin{itemize}[leftmargin=*]
%     \item At early rounds of running,  the estimate $q_{r-1}(\vectheta|\vecs_o)$ is often inaccurate. If we directly propose $\vectheta \sim q_{r-1}(\vectheta|\vecs_o)$, we would run the risk of focusing on a wrong region, especially when the mode of $q_{r-1}(\vectheta|\vecs_o)$ is away from that of the true posterior. By setting the high-density region of $q_{r-1}(\vectheta|\vecs_o)$ to be uniform, we reduce such risks, and still avoid exploring less-plausible regions;
%     \item At later rounds of learning, the region near the mode of $\pi(\vectheta|\vecs_o)$ is often learned accurately. In such cases, a better strategy to learn $\pi(\vectheta|\vecs_o)$ more accurately is to explore the region moderately away from the mode. Exploring the high-density region of  $q_{r-1}(\vectheta|\vecs_o)$ equally fits this goal. 
% \end{itemize}





% \begin{Proposition}
% Let the mode of the true posterior $\vectheta_* = \arg\max p(\vectheta|\vecx_o)$ be within the $\epsilon$-ball of the estimated mode: $\hat{\vectheta}_* = \arg\max \hat{p}(\vectheta|\vecx_o)$. Then we have better mass around $\vectheta_*$ with our prior.
% \end{Proposition}






% \section{Application}
% In this section, we further apply our automatic sufficient statistic approach to improve two popular likelihood-free algorithms: sequential Monte Carlo ABC [1], and sequential neural likelihood [2], yielding two new likelihood-free inference algorithms. In both algorithms, we adopt the same adaptive learning pipeline as aforementioned i.e we jointly learn the sufficient statistic $s(\cdot)$ and the posterior $\pi(\vectheta|\vecx_o)$ in multiple rounds. The difference lies in how they estimate  $\pi(\vectheta|\vecx_o)$ at each round.

















% \textbf{g-and-k} model. The last model we consider is 2D distribution widely used in quantitative finance. Data $\vecx$ from this model could be seen as generated by the following process:
% \[
%     \vecz \sim \mathcal{N}\Big(\vecz; \mathbf{0}, \begin{bmatrix}
%           1, & \lambda \\
%           \lambda, & 1\\
%          \end{bmatrix} \Big),
% \]
% \[
%      x_1 = Q(z_1; \vectheta), \qquad \qquad  x_2 = Q(z_2; \vectheta),
% \]
% \[
%     Q(z_d; \vectheta) = A_d + B_d\cdot \Big[1 + 0.8 \cdot \frac{1-e^{-g_d z_d}}{1+e^{-g_d z_d}} \Big] \cdot z_d(1+z_d)^2
% \]
% where $g_d >0$ and $k_d > -\frac{1}{2}$. Here, the parameters of interests are $\vectheta=\{A_1, g_1, B_2, k_2,\lambda \}$, and the true parameters are $\vectheta^*=\{A_1, g_1, B_2, k_2,\lambda \}$. This model does not has a analytical likelihood function since the inversion function: $z_d = Q^{-1}(x_d; \vectheta)$ does not has a closed form. However, we could still approximate the likelihood function numerically (e.g by inverting $Q$ with binary search). The true posterior is then approximated with this numerical likelihood.  




\textbf{M/G/1 queuing model}. This is a real-world problem describing the processing of incoming jobs in a single server system. Jobs in this model are served on a first-in-first-out (FIFO) basis, and subsequent job can not be processed until the previous job has finished. The data generating process in M/G/1 can be mathematically described as:
\[
\begin{split}
    s_i  &\sim \mathcal{U}(\theta_1, \theta_1 + \theta_2) \\
    v_i - v_{i-1} &\sim  \text{exp}(\theta_3) \\
    d_i - d_{i-1} &= s_i + \text{max}(0, v_i - d_{i-1})
\end{split}
\]
where $s_i$, $v_i$, $d_i$ are the service time, visiting time and finish time of job $i$ respectively. The parameters of interest in this problem are $\vectheta = ( \theta_1, \theta_2, \theta_3 )$ and the true parameter values are $\vectheta^* = ( 1.0, 4.0, 0.2 )$. The data $\vecx$ in this problem are the time intervals $x_i = d_i - d_{i-1}$ between the finish time of two consecutive jobs. 200 such intervals are observed so that $\vecx = \{x_1, \ldots, x_{200} \}$. Like in the Gaussian copula problem, we compute a rudimentary statistic for $\vecx$, and use this statistic in place of the original data in inference. Here, the statistic is taken as the 20 equally-spaced quantiles of $\vecx$. We then learn low-dimensional statistic from this rudimentary statistic with our method.

% \textbf{Lotka-Volterra problem}. The last problem we consider is a stochastic dynamical system in biology that describes predator-prey dynamics. There are four possible events in the system: (a) a predator being born, (b) a predator dying, (c) a prey being born, (d) a prey being eaten by the predator. The happening of these events can be probabilistically described as
% \begin{center}
% \begin{tabular}{ l l l}
%  $\text{Pr}(X \to X+1 | \vectheta) \propto \text{exp}(\theta_1) \cdot XY$ & $\quad$  & $\text{Pr}(Y \to Y+1 | \vectheta) \propto \text{exp}(\theta_3) \cdot Y$ \\ 
%  $\text{Pr}(X \to X-1 | \vectheta) \propto \text{exp}(\theta_2) \cdot X$
%   & $\quad$ & $\text{Pr}(Y \to Y-1 | \vectheta) \propto \text{exp}(\theta_1) \cdot XY$
% \end{tabular}
% \end{center}
% where $X, Y$ are the numbers of predators and preys respectively. The parameters of interest are $\vectheta = ( \theta_1, \theta_2, \theta_3 )$ and the true parameters are $\vectheta^* = ( \log(0.01), \log(0.5), \log(0.1) )$. The initial sizes of the populations are $(X^0, Y^0 ) =  (50, 100)$. While the likelihood is intractable, sampling from the model is relatively easy by e.g Gillspie’s algorithm \citep{g-algorithm}. We simulate the system for a total of 8 time units and record the values of $X$ and $Y$ after every 0.2 time units. This yields two time series of length 40 being our data. We then directly learn low-dimensional sufficient statistic from this data.

